Improving Robustness of Spectrogram Classifiers with Neural Stochastic Differential Equations

Signal analysis and classification is fraught with high levels of noise and perturbation. Computer-vision-based deep learning models applied to spectrograms have proven useful in the field of signal classification and detection; however, these methods aren't designed to handle the low signal-to-noise ratios inherent within non-vision signal processing tasks. While they are powerful, they are currently not the method of choice in the inherently noisy and dynamic critical infrastructure domain, such as smart-grid sensing, anomaly detection, and non-intrusive load monitoring.

==> 0_abstract.tex <==
%One of these challenges is confidently explaining signal classifications. 
Signal analysis and classification is fraught with high levels of noise and perturbation. Computer-vision-based deep learning models applied to spectrograms have proven useful in the field of signal classification and detection; however, these methods aren't designed to handle the low signal-to-noise ratios inherent within non-vision signal processing tasks. While they are powerful, they are currently not the method of choice in the inherently noisy and dynamic critical infrastructure domain, such as smart-grid sensing, anomaly detection, and non-intrusive load monitoring. %One of these challenges is confidently explaining signal classifications. 
\renewcommand{\thefootnote}{\fnsymbol{footnote}} 
Currently, these models can be brittle, which makes them susceptible to noisy input. This also means they have sub-optimal stability of explanation outputs. Experts and technicians using these models to make decisions in real world scenarios need assurance that a model is performing as it is supposed to.  The classification or prediction outputs it generates should be sound and grounded, not likely to change in the presence of shifting noise landscapes. In this work, we explore the idea of Neural Stochastic Differential Equations (NSDE's) to improve the robustness of models trained to classify time series data and the effect of NSDE's on the explainability of outputs. We then test the effectiveness of these approaches by applying them to a non-intrusive load monitoring (NILM) dataset that consists of simulated harmonic signals injected into a real building. \textcolor{white}{\footnote[2]{These author Equal Author Contribution}}
%We created an attribution-based confidence metric that can detect when the confidence in the outcome of neural network models trained on electromagnetic spectrograms is low and may require subject matter experts' (SME) intervention and/or automated model tuning. The goal is to ensure that the human SME relying on AI data-driven pipelines can develop a relationship of trust with robustly correct and well-calibrated neural networks.





==> 5_conclusion.tex <==
%One of these challenges is confidently explaining signal classifications. 
From our experiments, we show that a Neural-SDE variant of the ConvNext Res-Net architecture can provide improved robustness and attribution stability for spectrogram classification in the presence of signal noise, with minimal amounts of trade-off in accuracy. This relatively minor modification to the res-net architecture can provide benifits even in low-data-availability scenarios, as shown by using our relatively small dataset for training and testing. Additionally, with Neural-SDEs, IG and Noise tunneling can successfully identify the important signal features in STFT spectrogram images. Although these preliminary results are promising, accuracy rates in the presence of noise and adversarial input are still too low to be reliable. We hope to improve the efficacy of the NSDE method by investigating improved noise shaping and training augmentation schemes that could further bolster performace in low-data-availability or few-shot-learning settings.


==> backup.tex <==
\begin{figure}[h]
\centering
\label{fig:square75}
\includegraphics[width=0.45\textwidth]{figures/convNext.png}
\caption{Attribution range for \textcolor{red}{Add Type of image} image with \textcolor{red}{Add the frequency}}
\end{figure}

\begin{figure}[h]
\centering
\label{fig:triangle}
\includegraphics[width=0.45\textwidth]{figures/NeuralSDE.png}
\caption{Attribution range for \textcolor{red}{Add Type of image} image with \textcolor{red}{Add the frequency}}
\end{figure}

% https://medium.com/@kemalpiro/xai-methods-integrated-gradients-6ee1fe4120d8
% https://medium.com/@kemalpiro/xai-methods-noise-tunnel-31ca197fb560

%The \textit{Attribution-based Confidence (ABC)} metric \cite{jha2019attribution} serves to assess the reliability of deep neural network (DNN) outputs on input data. This method introduces an approach to estimate DNN prediction confidence utilizing attribution techniques such as IG to estimate the confidence level associated with DNN predictions. This is how they work together: Given an input sample $x$ to the DNN, IG is applied to compute the attribution map $A(x)$. This attribution map indicates the importance of each input feature in influencing the DNN's prediction for the input $x$. The ABC metric then calculates a confidence score $C(x)$ based on the attribution map $A(x)$ and the predicted class label $f(x)$. Here, the confidence score $C(x)$ represents the ratio of the sum of attribution scores associated with features relevant to the predicted class to the sum of all attribution scores across all features. A higher value of $C(x)$ indicates stronger agreement between the predicted class label and the salient features identified by IG, suggesting higher confidence in the prediction.


%ABC employs attribution-based dimensional reduction to identify locally relevant features near the input, eliminating the need for access to training data or additional calibration. The methodology entails computing attribution maps for each input sample, highlighting the significance of various features in the prediction process. Subsequently, a confidence score is derived based on the agreement between these attribution maps and the predicted class. A higher degree of concordance between the predicted class and the salient features identified in the attribution maps indicates greater confidence in the prediction's accuracy.

